Increasing the Efficiency of Cryptoasset Investigations by Connecting the Cases

Law enforcement agencies are confronted with a rapidly growing number of cryptoasset-related cases, often redundantly investigating the same cases without mutual knowledge or shared insights. In this paper, we explore the hypothesis that recognizing and acting upon connections between these cases can significantly streamline investigative processes. Through an analysis of a dataset comprising 34 cyberfraud and 1793 sextortion spam cases, we discovered that 41% of the cyberfraud and 96.9% of the sextortion spam incidents can be interconnected. We introduce a straightforward yet effective tool, which is integrated into a broader cryptoasset forensics workflow and allows investigators to highlight and share case connections. Our research unequivocally demonstrates that recognizing case connections can lead to remarkable efficiencies, especially when extended across crime areas, international borders, and jurisdictions.

==> macros-generic.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% generic macros

%----- Comments ----------------------------------------------------------------
\RequirePackage{totcount}
\RequirePackage{color}
%\RequirePackage[colorinlistoftodos]{todonotes}

%----- Table Column definitions 
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

\newcommand{\TODO}[1]{
  \if\relax\detokenize{#1}\relax
    \textcolor{red}{TODO}
  \else
    \textcolor{red}{ {#1}}
  \fi
}

% \newtotcounter{notecount}
% \newcommand{\notewarning}{%
% \ifnum\totvalue{notecount}>0%
%  \vspace{1ex}
% \begin{center}
%  \begin{tikzpicture}[baseline=(A.south)]
%     \node (A) [] at (0,0){};
%     \node [rounded corners=1pt,rectangle, draw=red, fill=red!20,text=black](B) at (0.1ex,0ex){
%         \Large \raggedright {\bf Warning:} There are still some notes left!
%     };
%  \end{tikzpicture}
% \end{center}
%  \vspace{1ex}
% \fi
% }
% \makeatletter
% \def\myaddcontentsline#1#2#3{%
%   \addtocontents{#1}{\protect\contentsline{#2}{#3}{Section \thesubsection\ at p. \thepage}{}}}

% \renewcommand{\@todonotes@addElementToListOfTodos}{%
%     \if@todonotes@colorinlistoftodos%
%         \myaddcontentsline{tdo}{todo}{{%
%             \colorbox{\@todonotes@currentbackgroundcolor}%
%                 {\textcolor{\@todonotes@currentbackgroundcolor}{o}}%
%             \ \@todonotes@caption}}%
%     \else%
%         \myaddcontentsline{tdo}{todo}{{\@todonotes@caption}}%
%    \fi}%

% \newcommand*\mylistoftodos{%
%   \begingroup
%        \setbox\@tempboxa\hbox{Section 9.9 at p. 99}%
%        \renewcommand*\@tocrmarg{\the\wd\@tempboxa}%
%        \renewcommand*\@pnumwidth{\the\wd\@tempboxa}%
%        \listoftodos%
%   \endgroup
% }
% \makeatother
% \definecolor{lightgreen}{rgb}{0.86, 0.93, 0.78}
% \definecolor{bordergreen}{rgb}{0.55, 0.76, 0.74}
% \definecolor{lightblue}{rgb}{0.70, 0.90, 0.99}
% \definecolor{borderblue}{rgb}{0.01, 0.66, 0.96}
% \definecolor{lightamber}{rgb}{1, 0.93, 0.70}
% \definecolor{borderamber}{rgb}{1, 0.76, 0.03}
% \definecolor{lightcolor4}{rgb}{ 0.93, 0.70, 1}
% \definecolor{bordercolor4}{rgb}{0.76, 0.03, 1}

% %\newcommand{\note}[1]{\stepcounter{notecount}\todo[inline,bordercolor=bordergreen,linecolor=bordergreen,color=lightgreen]{ #1}{}}
% %\newcommand{\snote}[1]{\stepcounter{notecount}\todo[bordercolor=bordergreen,linecolor=bordergreen,color=lightgreen,fancyline]{ #1}{}}

% \newcommand{\anote}[1]{
%   \stepcounter{notecount}
%   \todo[
%         inline,
%         caption={minipage-note},
%         bordercolor=bordergreen,
%         linecolor=bordergreen,
%         color=lightgreen,
%         fancyline
%       ]
%       {
%         \begin{minipage}{0.9\textwidth}
%            #1
%         \end{minipage}
%       }
%       {}
% }

% \newcommand{\TODO}[1]{
%   \if\relax\detokenize{#1}\relax
%     \textcolor{red}{TODO}
%   \else
%     \textcolor{red}{ {#1}}
%   \fi
% }

% \newcommand{\footTODO}[1]{\footnote{\TODO{#1}}}

% %----- Boxed figures ----------------------------------------------------------------

% \newenvironment{boxfig}[2]{% {#1}{#2} = {Figure Caption}{label}
%   \begin{figure}[t!]
%     \newcommand{\FigCaption}{#1}
%     \newcommand{\FigLabel}{#2}
%     \begin{center}
%       \begin{small}
%       \setlist{nosep}
%         \begin{tabular}{@{}|@{~~}l@{~~}|@{}}
%           \hline
%           \rule[-1.5ex]{0pt}{1ex}
%           \begin{minipage}[b]{0.96\linewidth}
%             %\smallskip
%              \caption{\FigCaption}
%              \label{\FigLabel}
%              \medskip
%             }{%
%           \end{minipage}\\
%           \hline
%         \end{tabular}
%       \end{small}
%     \end{center}
%   \vskip -8mm
%   \end{figure}
% }

% %----- Box Environment ---------------------------------------------------------

% \RequirePackage{mdframed}

% %Basic box structure with title box
% \newenvironment{titlebox}[3]
%  {\mdfsetup{
%    style=#2,
%    innertopmargin=1.1\baselineskip,
%    skipabove={\dimexpr0.7\baselineskip+\topskip\relax},
%    skipbelow={1em},needspace=3\baselineskip,
%    singleextra={\node[#3,right=10pt,overlay] at (P-|O){~{\sffamily\bfseries #1 }};},%
%    firstextra={\node[#3,right=10pt,overlay] at (P-|O) {~{\sffamily\bfseries #1 }};},
%    frametitleaboveskip=9em,
%    innerrightmargin=5pt
%   }
%   \begin{mdframed}[font=\small]\setlist[itemize]{leftmargin=13pt}\setlist[enumerate]{leftmargin=13pt}\raggedright% 
%  }
%  {\end{mdframed}}

%  %title box style
%  \tikzstyle{normal} = [thick, fill=white, text=black, draw, rounded corners, rectangle, minimum height=.7cm, inner sep=3pt]
%  \tikzstyle{gray} = [thick, fill=gray!90, text=white, rounded corners, rectangle, minimum height=.7cm, inner sep=3pt]

% \newenvironment{boxfig2}[2]
% {
%   %\begin{figure}[t!]
%     \begin{titlebox}{{#1}}{commonbox}{normal}
%   \begin{small}
%   \setlist{nosep}
% }
% {
%   \end{small}
%   \end{titlebox}
%   %\end{figure}
% }

% %----- Generic notation ----------------------------------------------------------------

% \newcommand{\eqdef}{\triangleq}
% \newcommand{\defeq}{\eqdef}

% \newcommand{\bits}{\{0,1\}}
% \newcommand{\bin}[1]{\ensuremath{\{0,1\}^{#1}}}
% \newcommand{\concat}{\,\|\,}
% \newcommand{\eps}{\varepsilon}
% \newcommand{\rsample}{\stackrel{\mbox{\tiny $\$$}}{\leftarrow}}

% %check and cross marks
% %\usepackage{pifont}% http://ctan.org/pkg/pifont
% \newcommand{\cmark}{\ding{51}}%
% \newcommand{\xmark}{\ding{55}}% 

% % brackets
% \newcommand{\ngroup}[1]{\left(#1 \right)}
% \newcommand{\sgroup}[1]{\left[#1 \right]}
% \newcommand{\cgroup}[1]{\left\{#1 \right\}}
% \newcommand{\agroup}[1]{\left\langle #1 \right\rangle}

% \newcommand{\Prob}[1]{\Pr\left[#1 \right]}
% \newcommand{\CondProb}[2]{ \Prob{#1 \,\big|\, #2}}
% \newcommand{\Exp}[1]{\mathsf{E}\left[#1\right]}
% \newcommand{\CondExp}[2]{\Exp{#1\,|\,#2}}
% \newcommand{\abs}[1]{\left| #1 \right|}
% \newcommand{\setd}[2]{\left\{ #1 \,:\, #2 \right\}}

% %----- Other ----------------------------------------------------------------

% \newcommand{\ignore}[1]{}

% \makeatletter
% \newcommand\parag{%
%    \@startsection{paragraph}{4}{\z@}%
%        {-3\p@ \@plus -1\p@ \@minus -1\p@}%
%        {-0.2em \@plus -0.12em \@minus -0.05em}%
%        {\normalfont\normalsize\scshape}}
% \newcommand{\heading}[1]{\parag{#1}}
% \makeatother 



